Analyzing and Improving Neural Networks by Generating Semantic Counterexamples through Differentiable Rendering

Even as deep neural networks (DNNs) have achieved remarkable success on vision-related tasks, their performance is brittle to transformations in the input. Of particular interest are semantic transformations that model changes that have a basis in the physical world, such as rotations, translations, changes in lighting or camera pose. In this paper, we show how differentiable rendering can be utilized to generate images that are informative, yet realistic, and which can be used to analyze DNN performance and improve its robustness through data augmentation. Given a differentiable renderer and a DNN, we show how to use off-the-shelf attacks from adversarial machine learning to generate semantic counterexamples -- images where semantic features are changed as to produce misclassifications or misdetections. We validate our approach on DNNs for image classification and object detection. For classification, we show that semantic counterexamples, when used to augment the dataset, (i) improve generalization performance (ii) enhance robustness to semantic transformations, and (iii) transfer between models. Additionally, in comparison to sampling-based semantic augmentation, our technique generates more informative data in a sample efficient manner.

==> Macros/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> NeurIPS/2_related_work.tex <==
%\section{Related Work}
\subsection*{Related Work}
\label{sec:related}

\sanjit{Merged this into Introduction as a subsection. Need to also discuss GANs or other generative methods for producing `realistic' images modifications}

{\bf Inverse Graphics:} The process of finding 3D scene parameters (geometric, textural, lighting, etc.) given images is referred to as de-rendering or inverse graphics~\cite{Baumgart, Faces, AutoLighting, Shape}. Pipelines for differentiable rendering (the opposite of inverse graphics) were proposed by Loper \etal~\cite{Loper} and Kato \etal~\cite{Kato}.
Kulkarni \etal~\cite{kulkarni2015deep} combine both de-rendering and rendering, and propose a model that learns interpretable representations of images (similar to image semantics), and show how these interpretations can be modified to produce changes in the input space. Li \etal~\cite{li2018differentiable} design a general-purpose differentiable ray tracer; gradients can be computed with respect to arbitrary semantic parameters such as camera pose, scene geometry, materials, and lighting parameters. Similarly, Yao \etal~\cite{3dsdn2018} propose a pipeline that, through de-rendering obtains various forms of semantics, geometry, texture, and appearance, which can be rendered using a generative model. 
\sanjit{Say explicitly that we use the DRs of Li et al and Yao et al.?}

{\bf Adversarial Examples:} By construction, adversarial examples are test-time inputs that result in incorrect outputs produced by the ML model. Extensive prior work~\cite{Madry,FGSM,carlini2017towards,moosavi2016deepfool,papernot2016limitations} focuses on generating norm-bounded pixel-level changes to input features to induce incorrect actions. However, these manipulations are not easily realizable in the real world. Generating real world adversarial examples has resulted in several efforts~\cite{athalye2017synthesizing,eykholt2018robust,bhattad2020unrestricted}, some of which are more realistic than others. We will restrict our focus to those attacks that result in {\em semantically meaningful} adversarial samples. For example, Geirhos \etal~\cite{Texture} discovered that certain models are biased towards textural cues, while Engstrom \etal~\cite{engstrom2019exploring} observe that modifying the spatial orientation of images results in misclassifications. Sharif \etal~\cite{sharif2016accessorize} create semantic attacks against facial recognition systems by {\em realizing} changes in pixel intensities by placing brightly colored objects on faces. Approaches involving explicitly sampling the semantic parameter space are slow and expensive~\cite{SAESeshia}. Work that is closest to ours is that of Xiao \etal~\cite{Xiao_2019_CVPR} and Qiu \etal~\cite{SemanticAdv}. The former uses a differentiable renderer to induces changes in shapes and textures, while the latter induces a different set of semantic changes using a generative model. 






==> NeurIPS/3_overview.tex <==
\section{Semantic Adversarial Examples}
\label{sec:sae}

Consider a space $Z$ of the form $X \times Y$, where $X$ is the sample space and $Y$ is the set of labels. From here on we will assume that $X = \Real^n$.  Let $H$ be a hypothesis space (\eg weights of a DNN). We assume a loss function $\ell: H \times Z \mapsto \Real$ so that given a hypothesis $w \in H$ and a labeled data point $(x,y) \in Z$, the loss is $\ell(w,x,y)$.  The output of the learning algorithm is a {\em classifier}, which is a function from $\Real^n$ to $Y$. To emphasize that a classifier depends on a hypothesis $w \in H$, which is output of the learning algorithm, we will denote it as $F_w$ (if $w$ is clear
from the context, we will sometimes simply write $F$). The "softmax" output corresponding the classifier $F$ is denoted by $s(F)$ and is a function
from $X \rightarrow \Delta (Y)$, where $\Delta(Y)$ is the set of distributions over $F$. Typically, $F(x)$ is defined as $\argmax_{y \in Y} s(F)(y)$

The rest of the section is organized as follows: Subsection~~\ref{trad} provides an overview of adversarial examples (reader familiar
with the literature can skip this section). Subsection~~\ref{transformation} presents the concept of semantic transformation, which is used in subsection~~\ref{sae}
to describe semantic adversarial examples. 

\subsection{Traditional Adversarial Examples}
\label{trad}

We will focus our discussion on untargeted attacks, but our discussion also applies to targeted attacks.  An adversary $A$'s goal is to take any input vector $\bfx \in \Real^n$ and produce a minimally altered version of $\bfx$, an \emph{adversarial example} denoted by $A(\bfx)$, that has
the property of being misclassified by a classifier $F : \Real^n
\rightarrow Y$. The adversary wishes to solve the following optimization problem:

\[
\begin{array}{lr}
\min_{\bfdelta \in \Real^n}  & \mu ( \bfdelta ) \\
\mbox{such that} & F( \bfx + \bfdelta ) \not= F(\bfx) 
\end{array}
\]
The various terms in the formulation are: $\mu$ is a norm on $\Real^n$; $\mu$ can be $l_\infty$, $l_0$, $l_1$, or $l_p$ ($p \geq 2$). While not representative, these norms are commonly used as an approximation of a human's visual perception~\cite{sen2019should}. If $\bfdelta$ is the solution of the optimization problem given above, then the adversarial example $A(\bfx) \; = \; \bfx+\delta$.

\noindent\textbf{FGSM:} The \emph{fast gradient sign method (FGSM)}~\cite{FGSM} was one of the first untargeted attacks developed in literature. The adversary crafts an adversarial example for a given legitimate sample $\bfx$ by computing (and then adding) the following perturbation:
\begin{equation}
\label{eq:goodfellow-perturbation}
\bfdelta  = \varepsilon \signf(\nabla_{\bfx} L_F (\bfx))
\end{equation}

%The adversarial example $A(\bfx)$ is $\bfx+\bfdelta$.  
The function $L_F (\bfx)$ is a shorthand for $\ell (w,\bfx,l(\bfx))$, where $w$ is the hypothesis corresponding to the classifier $F$, $\bfx$ is the data point and $l(\bfx)$ is the true label of $\bfx$ (essentially we evaluate the loss function at the hypothesis corresponding to the classifier). The gradient of the function $L_F$ is computed with respect to $\bfx$
using sample $\bfx$ and label $y = l(\bfx)$ as inputs. Note that
$\nabla_{\bfx} L_F (\bfx)$ is an $n$-dimensional vector and
$\signf(\nabla L_F (\bfx))$ is a $n$-dimensional vector whose $i^{th}$ element is the sign of  $ \nabla_{\bfx} L_F (\bfx) [i]$.  The value of the \emph{input variation parameter} $\varepsilon$ factoring the sign matrix controls the perturbation's amplitude. Increasing its value increases the likelihood of $A(\bfx)$ being misclassified by
the classifier $F$ but also makes adversarial examples
easier to ``detect'' by humans. The key idea is that FGSM takes a step {\it in the direction of the gradient of the loss function with respect to the input}, thus attempting to maximize the loss function using its first-order approximation. Recall that stochastic gradient descent (SGD) takes a step in the direction that is on expectation opposite to the gradient of the loss function because it is trying to minimize the loss function.

\noindent\textbf{PGD:} In \emph{Projected Gradient Descent (PGD)}~\cite{Madry}, we find a perturbation in an iterative manner. The PGD attack can be thought of an iterative version of FGSM. Assume that we are using the $l_p$ norm. Assume $\bfx_0$ is the original sample $\bfx$.
\begin{equation}
\label{eq:PGD}
\bfx_{k+1}  = \Pi_{B_p (\bfx,\varepsilon)} (\bfx_k + \varepsilon \signf(\nabla_{\bfx} L_F (\bfx) ))
\end{equation}

The operator $\Pi_{B_p (\bfx,\varepsilon)} (y)$ is the projection
operator, \ie it takes as input a point $y$ and outputs the closest
point in the $\varepsilon$-ball (using the $l_p$-norm) around
$\bfx$. The iteration stops after a certain number of steps (the
exact number of steps is a hyperparameter).

%added in by lakshya
\noindent\textbf{Carlini-Wagner:} In the \emph{Carlini-Wagner}~\cite{carlini2017towards} attack algorithm, the perturbation distance metric $D(x,x+\delta)$ is minimized subject to $f(x+\delta) \leq 0$ and $x+\delta \in [0,1]^n$, where $f(x)$ is a function indicating whether or not the desired misclassification has been achieved. The formulation can thus be simplified to 
\begin{equation}
    \min \| \delta \|_p + c \cdot f(x + \delta)
    \text{ such that } x+\delta \in [0,1]^n
\end{equation}
For the purposes of our attack, we use the 2-norm in our distance metric. 

\subsection{Semantic Transformation}
\label{map}
We assume that there is a {\it semantic transformation} $\tau: (\Real^n \times \Theta) \rightarrow \Real^n$.
Moreover, we assume$\mu$ is a norm over $\Theta$. The reader can think of $\Theta$ as parameters that control the transformations (\eg the angle of rotation). Given $\theta \in \Theta$, $\tau(x,\theta)$ is the image transformed according to the parameters $\theta$. We assume that there is a special identity element in $\Theta$ (which we call $\perp$) such that $\tau(\bfx,\perp) = \bfx$. We assume that $\tau(x,\theta)$ is differentiable in $\theta$.
We also assume that there is an operator $\oplus$ called the aggregation 
operator (similar to addition in $\Real^n$), but in the parameter
space $\Theta$. The precise axioms satisfied by $\oplus$ depends
on $\Theta$, but one axiom we require in our construction is the following:
\begin{eqnarray*}
\tau(\bfx, \bftheta_1 \oplus \bftheta_2) & = & 
\tau(\tau(\bfx,\bftheta_1),\bftheta_2)
\end{eqnarray*}


{\bf Differentiable rendering and inverse graphics.} One way to create a semantic transformation is
to use a differentiable renderer/de-renderer in an inverse graphics setting (see Figure~\ref{fig:DR}). Such an inverse graphics setting can be thought of two transformations: (a) a de-renderer $\beta : \Real^n \rightarrow \mathcal{S}$, and (b) a renderer $\gamma: \mathcal{S} \rightarrow \Real^n$. Here, $\mathcal{S}$ is the intermediate representation (IR). In the differentiable renderer/de-renderer we utilize~\cite{3dsdn2018}, the IR contains a semantic map, texture codes, and 3D attributes. Let $\Theta$ be the set of 
parameters that can be changed in the IR (\eg change to the texture code to make it more cloudy) and $\perp \in \Theta$ corresponds to the identity. Suppose there is an
operator $\alpha : (\mathcal{S} \times \Theta) \rightarrow
\mathcal{S}$ that given a $\theta \in \Theta$ transforms the IR, \ie $\alpha(s,\theta)=s'$ for $s,s' \in \mathcal{S}$. In this
case, the function $\tau (\bfx,\theta)$ is equal to
$\gamma(\alpha(\beta(\bfx),\theta))$. We use the fact that for
differentiable renderers/de-renderers the functions $\beta$, $\gamma$, $\alpha$ are differentiable.

\begin{figure}[!h]
\centering
\includegraphics[width=0.8\textwidth]{figures/pipeline.png}
\caption{\varun{need new figure}The input is de-rendered (step 1) to its intermediary representation (IR) - semantic, graphic, and textural maps. Then, this is adversarially perturbed (\eg the red car is rotated) as described in \S~~\ref{sae} (step 2). The resulting IR is then re-rendered to the generate the SAE (step 3).}
\label{fig:DR}
\end{figure}


\subsection{Semantic Adversarial Examples (SAEs)}
\label{sae}
Throughout this section we assume that there is a semantic transformation $\tau: (\Real^n \times \Theta) \rightarrow \Real^n$ that is 
differentiable in $\theta$. An adversarial attack in this context can be formalized as follows:  

\[
\begin{array}{lr}
\min_{\theta \in \Theta}  & \mu ( \theta ) \\
\mbox{such that} & F(\tau (\bfx,\theta)) \not= F(\bfx) 
\end{array}
\]


In other words, we ideally want to find a ``small perturbation'' in the parameter space $\Theta$ that will misclassify the sample\footnote{\textcolor{blue}{However, the existence of such a function for the semantic space is an open research question; the semantic parameter space is not homogeneous and it is unclear if one function can be used to capture the distance amongst all these transformations. Not only should the norm measure the changes in the semantic space, it should also approximate human perception. In its presence, one would be able to effectively measure the distortion introduced by the adversary in the semantic space.}}. 

Let $A(F,\bfx)$ be an attack algorithm to generate traditional adversarial examples (see Subsection~\ref{trad}). We 
outline a general technique for transforming $A$ to $sA$ that generates semantic adversarial examples. The technique
works as by transforming algorithm $A$ using the following rules:
\begin{itemize}
\item Replace $\bfdelta$ with $\theta$.
\item Replace $\bfx+\bfdelta$ with $\tau(\bfx,\theta)$.
\item Use chain rule to compute the gradients of terms, such as loss function, that involve $\tau(\bfx,\theta)$.
\end{itemize}
Consider the function $L_F (\tau (\bfx,\theta))$.
%The derivative with respect to $\theta$ is $\nabla_{\bfz} L_F (\bfz) |_{\bfz = \tau(\bfx, \perp)} \nabla_{\theta} \tau(\bfx,\theta)$ (the notation $\nabla_{\bfz} L_F(\bfz) |_{\bfz = \tau(\bfx, \perp)}$ is the derivative evaluated at $\tau(\bfx, \perp)$).
The derivative with respect to $\theta$ is $\left.\left[\frac{\partial\tau}{\partial\theta}\right]^{\top}\right\vert_{\bfx}\left.\nabla_{\bfz} L_F (\bfz)\right\vert_{\bfz = \tau(\bfx, \theta)}$ (the notation $\left.\left[\frac{\partial\tau}{\partial\theta}\right]^{\top}\right\vert_{\bfx}$ is the transposed Jacobian matrix of $\tau$ as a vector-valued function of $\theta$, evaluated at $\bfx$, and  $\nabla_{\bfz} L_F(\bfz) |_{\bfz = \tau(\bfx, \theta)}$ is the derivative evaluated at $\tau(\bfx, \theta)$). The semantic version of FGSM ({\it sFGSM}) will produce the following $\bftheta$:

\begin{equation}
\label{eq:sFGSM}
\bftheta^\star  = \varepsilon \signf\left(\left.\left[\tfrac{\partial\tau}{\partial\theta}\right]^{\top}\right\vert_{(\bfx, \perp)}\left.\nabla_{\bfz} L_F (\bfz) \right|_{\bfz = \tau(\bfx, \perp)}\right)
\end{equation}

% \begin{equation}
% \label{eq:sFGSM}
% \bftheta^\star  = \varepsilon \signf(\nabla_{\bfz} L_F (\bfz) |_{\bfz = \bfx} \nabla_{\theta} \tau(\bfx,\theta)) |_{\theta = \perp}
% \end{equation}

The adversarial example $A(\bfx)$ is $\tau(\bfx,\bftheta^\star)$. Note that we do not assume any special properties about $\tau$, such as  linearity. We only assume that $\tau$ is differentiable. %, which get because of the user of differentiable rendering. 

In a similar manner a semantic version of the PGD attack ({\it sPGD}) can be constructed.  Let $\bftheta_0 = \perp$ and $\bfx_0 = \bfx$. The update steps correspond to the following two equations:
\begin{eqnarray*}
  \bftheta_{k+1}  & = & \Pi_{B_\mu (\bftheta_0,\varepsilon)}
  \left(\bftheta_k \; \oplus \;
  \varepsilon \signf\left(\left.\left[\tfrac{\partial\tau}{\partial\theta}\right]^{\top}\right\vert_{(\bfx_k, \theta_k)}\left.\nabla_{\bfz} L_F (\bfz) \right|_{\bfz = \tau(\bfx_k, \theta_k)}\right)\right) \\
  \bfx_{k+1} & = & \tau (\bfx_0,\bftheta_{k+1})
\end{eqnarray*}


% \begin{eqnarray*}
%   \bftheta_{k+1}  & = & \Pi_{B_\mu (\bftheta_0,\varepsilon)}
%   (\bftheta_k \; \oplus \;
%   \varepsilon \signf(\nabla_{\bfz} L_F (\bfz) |_{\bfz = \bfx} \nabla_{\theta} \tau(\bfx_k,\theta) |_{\theta = \bftheta_k}) ) \\
%   \bfx_{k+1} & = & \tau (\bfx_0,\bftheta_k)
% \end{eqnarray*}
Note that $\Pi_{B_\mu (\cdot,\cdot)}$ is the projection operator in the parameter space $\Theta$. We also assume that the 
projection operator will keep the parameters in the feasible 
set, which depends on the image (\eg translation does not take the 
car off the road). 

Even though we only considered semantic versions of FGSM, Carlini-Wagner, and PGD, our technique can be used to transform any attack algorithm.
% such as Carlini \& Wagner~\cite{carlini2017towards} 
% that adds a perturbation $\bfdelta$, to its ``semantic version''. 


 






==> NeurIPS/4_information.tex <==
\section{Augmentation Quality}
\label{sec:quality}

Various strategies, such as random sampling in the semantic parameter space, can be utilized to generate  samples
for augmentation. Suppose there is a dataset $D$ and we have two examples for augmentation $(x,y)$ and 
$(x',y')$. Which one is better for augmentation?
In this section, we formalize the notion of {\em informativeness} of address
this question. More details and intuitions about our metric appears in in Appendix~\ref{notes_augmentation}.

\subsection{Entropy \& Information Worth}
\label{entropy}

A common measurement that is used to measure the {\em goodness} of a classifier's predictive capabilities makes use of the concept of Shannon entropy~\cite{shannon, quinlan} which measures the unpredictability of outcome from a given set.
Let the label set $Y$ have $L$ labels $\{l_1,\cdots, l_L \}$.
Given set of datapoints $D=\{(x_1, y_1),\cdots, (x_m, y_m)\}$ where $y_t\in Y$ is the true label of a point $x_t$, a classifier $F$ on the set $D$ divides the set into subsets $D_1, \ldots, D_L$ where $D_i$ contains points whose predicted label is $l_i$. Let $E_i$ be the entropy measured on each subset $D_i$ of size $m_i$ \ie $E_i = -\sum_{j\in L} p_j^i\log p_j^i$, where $p_j^i$ is the estimated probability of observing the class $j$ in the subset $D_i$.

%(in the equation given below $m_i=|D_i|$)

\begin{align*}
    p_j^i = \frac{\sum_{t=1}^{m_i} \mathds{1}[x_t\in D_i] \mathds{1}[y_t=j]}{m_i} = \frac{\sum_{t=1}^{m_i} \mathds{1}[f(x_t)=i] \mathds{1}[y_t=j]}{m_i}
\end{align*}

If the entropy $E_i$ for each subset $D_i$ is low, then the classifier divides $D$ in a "well-organized" way, \ie the subset is extremely likely to consist of datapoints of single label. Thus, the following weighted average of $E_i$'s (henceforth referred to as {\em information worth}) is used to estimated the quality of a classifier \ie  $\hat E = \sum_{i\in[N]}\alpha_i \cdot E_i$, where each weight $\alpha_i$ is determined by the proportion of the size of the subset $D_i$ to the size of the entire set $D$ \ie $\alpha_i = \frac{|D_i|}{|D|} = \frac{m_i}{m}$. 

%(this is reminiscent of importance sampling).

We also want to make use $\hat E$ as a measure of the quality of augmented data. As long as the datapoints used for augmentation are realistic, it is better to have datapoints that do not agree with the current classifier, as we expect the re-training to improve the classifier by fixing the incorrect classification. Therefore, the datapoints that will increase the value of $\hat E$ after adding them to existing dataset (\ie augmentation) are desirable. We specify a more precise definition of information worth (the one we use in our evaluation) that incorporates realism in Appendix~\ref{generalization}.

\subsection{A Generalization Of The Definition}
\label{generalization}

The previous definition of $\hat E$ depends only on the predictions of the classifier. Thus, it is hard to distinguish between augmenting samples generated using the methodology defined in \S~\ref{map} from those generated using random sampling, for example. However, one may prefer a counterexample for which the classifier has a lower confidence, as it captures its {\em badness}, or one that is more {\em realistic}.

% \noindent{\bf Step 1: Incorporating Classifier Confidence.} Instead of considering the division of the set $D$ into subsets $D_1, \ldots, D_N$, we consider the division of the set $D$ into subsets $(D,\mu_1), \ldots, (D, \mu_N)$ where $\mu_i$ is the membership function of the $i^{th}$ subset, \ie $\mu_i(x)$ denotes how much $x$ belongs to $i$-th subset $(D,\mu_i)$. While $\mu_i$'s can be defined in various ways depending on the application, we choose the most natural choice of membership function $\mu_i(x) = s(F)(x)_i$ which denotes the softmax value of $x$ for class $i$.

% Consider the division of the set $D$ into subsets $(D,\mu_1), \ldots, (D, \mu_N)$ where $\mu_i$ is the membership function of the $i^{th}$ subset, \ie $\mu_i(x)$ denotes the probability with which $x$ belongs to the $i$-th subset $(D,\mu_i)$. 

\noindent{\bf Incorporating Classifier Confidence \& Realism.} In the previous definition, each point $x$ could belong to only 1 subset. However, with most DNN-based models, a point could belong to many classes (and consequently subsets) depending on its softmax values. Thus, let $\mu_i(x)$ denote the membership of a point to subset $i$. The most natural choice of $\mu_i(x) = s(F)(x)_i$ which denotes the softmax value of $x$ for class $i$. We also assume that there exists a quantifiable measure of realism $\rho$ such that $\rho(x)\in [0,1]$ (larger value means the image is more realistic). In this work, since we generate a new datapoint $x'$ from a reference datapoint $x^*$, we first define the similarity $\sigma$ of $x'$ to $x^*$ as $\sigma(x'; x^*) = 1 - \frac{d(x', x)}{d_\text{max}}$, where $d$ is the LPIPS distance~\cite{lpips} and $d_\text{max}$ is the maximum LPIPS score achievable. This metric assigns $\rho(x^*;x^*)=1$, because when there is no perturbation, \ie $x'=x^*$, then $d(x^*,x^*) = 0$. Therefore, we define $\rho(x)$ for $x\in S$ as 
$\sigma (x; x^*)$. Since $\rho$ captures {\em realism}, if the value $\rho(x)$ is small for some data point $x$, we do not trust the classification result $F(x)$. Based on this intuition, we control the participation of each datapoint $x$ in the information worth calculation by weighting it by its realism $\rho(x)$.  These ideas are captured by using the following $p_j^i$ and $\alpha_i$.

\begin{align*}
    p_j^i &= \frac{\sum_{t=1}^m \rho(x_t)\mu_i(x_t)\mathds{1}[y_t=j]}{\sum_{l\in[N]}\sum_{t=1}^m \rho(x_t)\mu_i(x_t)\mathds{1}[y_t=l]} = \frac{\sum_{t=1}^m \rho(x_t)\mu_i(x_t)\mathds{1}[y_t=j]}{\sum_{t=1}^m \rho(x_t)\mu_i(x_t)}\\
    \alpha_i &= \frac{\sum_{t=1}^m \rho(x_t)\mu_i(x_t)}{\sum_{l\in[N]}\sum_{t=1}^m \rho(x_t)\mu_i(x_t)}
\end{align*}


% \iffalse
% The previous definition of $\hat E$ depends only on the predictions of the classifier. Thus, it is hard to distinguish between augmenting samples generated using the methodology defined in \S~\ref{map} from those generated using random sampling, for example. However, one may prefer an augmentation sample for which the classifier has a lower confidence, as it captures its {\em badness}, or one that is more {\em realistic}. The confidence of the classifier on a point $x$ and label  $l_i$ is given by $s(F)(x)_i$ (recall that $s(F)(\cdot)$ is the softmax output corresponding to the classifier $F$). For brevity, we denote this as $\mu_i(x)$

% \paragraph{Incorporating Realism.} We assume that there exists a quantifiable measure of realism $\rho$ such that $\rho(x)\in [0,1]$ (larger value means the image is more realistic). In this work, since we generate a new datapoint $x'$ from a reference datapoint $x^*$, we first define the similarity $\sigma$ of $x'$ to $x^*$ as $\sigma(x'; x^*) = 1 - \frac{d(x', x)}{d_\text{max}}$, where $d$ is the LPIPS distance~\cite{lpips} and $d_\text{max}$ is the maximum LPIPS score achievable. This metric assigns $\rho(x^*;x^*)=1$, because when there is no perturbation, \ie $x'=x^*$, then $d(x^*,x^*) = 0$. Therefore, we define $\rho(x)$ for $x\in S$ as 
% $\sigma (x; x^*)$. Since $\rho$ captures {\em realism}, if the value $\rho(x)$ is small for some data point $x$, we do not trust the classification result $F(x)$. Based on this intuition, we control the participation of each datapoint $x$ in the information worth calculation by weighting by its realism $\rho(x)$. 

% These ideas are captured by using the following $p_j^i$ and $\alpha_i$ in our metric $\hat E$.

% \begin{align*}
%     p_j^i &= \frac{\sum_{t=1}^m \rho(x_t)\mu_i(x_t)\mathds{1}[y_t=j]}{\sum_{l\in[N]}\sum_{t=1}^m \rho(x_t)\mu_i(x_t)\mathds{1}[y_t=l]} = \frac{\sum_{t=1}^m \rho(x_t)\mu_i(x_t)\mathds{1}[y_t=j]}{\sum_{t=1}^m \rho(x_t)\mu_i(x_t)}\\
%     \alpha_i &= \frac{\sum_{t=1}^m \rho(x_t)\mu_i(x_t)}{\sum_{l\in[N]}\sum_{t=1}^m \rho(x_t)\mu_i(x_t)}
% \end{align*}

% \fi

==> NeurIPS/5_implementation.tex <==
\section{Implementation}
\label{sec:implementation}

%\sanjit{Merge with Evaluation section?}

For our experiments, we utilize two differentiable graphics frameworks: (i) 3D-SDN proposed by Yao \etal~\cite{3dsdn2018}, and (ii) Redner proposed by Li \etal~\cite{li2018differentiable}. The former comprises an inverse graphics and differentiable renderer; the latter comprises just a differentiable renderer. Using these frameworks, we augment two popular synthetic datasets: (i) VKITTI~\cite{vkitti}: scenes from photo-realistic proxy virtual worlds used for multi-object tracking, and (ii) ShapeNet~\cite{chang2015shapenet}: 
a large-scale repository of shapes represented by 3D CAD models of objects, organized under the WordNet taxonomy. We utilize the former dataset in the context of object detection with SqueezeDet~\cite{squeezedet} as our target model, and the latter for image classification using VGG-16~\cite{vgg} and ResNet-50~\cite{resnet} as target models.

We generate \SAEs by modifying elements from 2 popular attacks -- i-FGSM~\cite{FGSM} (iterative FGSM) and CW~\cite{carlini2017towards}  -- to generate their semantic counterparts. We also formulate a custom attack based on gradient descent (henceforth referred to as GD). Our implementation with 3D-SDN involves 1000 lines of code; this involves making changes to the original code to enable end-to-end differentiation, and replacing several image manipulations with their differentiable counterparts. Our implementation with Redner~\cite{li2018differentiable} involves 618 lines of code. The code is available at \url{https://anonymous.4open.science/r/1766a57c-d61f-42e4-aea1-f19fa5f0bc37/}\footnote{We can not open source the code using 3D-SDN as we do not own the license for the code.} We compare these \SAEs with augmenting samples generated using (i) random sampling, and (ii) Halton sampling~\cite{halton,dreossi-ijcai18} as baselines. All \SAEs generated involve modifying multiple semantic parameters (refer \S~\ref{combinations} in the Appendix for more details). More details, such as the exact hyperparameters used for our generation process (and for the baselines), the semantic parameters modified, the size of the datasets, model parameters etc. are presented in Appendix~\ref{specifics_implementation}.



==> NeurIPS/community.tex <==
\section*{Community Impact Statement}

Machine Learning (ML) models, such as deep neural networks (DNNs), have shown remarkable success for several vision-related tasks -- sometimes beating human performance. Thus, ML models have started being used in safety-critical scenarios. One such safety-critical application is the use of  ML models in control loops in cyber-physical systems (CPS), such as autonomous driving vehicles and drones. As evidenced by several real-world incidents, brittleness of ML models in CPS can have disastrous consequences.

The broader impact of this work is to bring higher assurance to the ML components of a control loop in a safety-critical CPS.  In particular, this work presents a systematic methodology to make these
components more robust to semantic changes in the environment being perceived by
the ML models. These are changes in position, orientation, color, texture, time of day,
weather conditions, camera pose, etc. which correspond to physically realizable
modifications in the environment. Safety-critical CPS must be robust to such changes
in order for their use in societally-important applications in transportation,
healthcare, and infrastructure. 


